A Uniform Treatment of Aggregates and Constraints in Hybrid ASP

Characterizing hybrid ASP solving in a generic way is difficult since one needs to abstract from specific theories. Inspired by lazy SMT solving, this is usually addressed by treating theory atoms as opaque. Unlike this, we propose a slightly more transparent approach that includes an abstract notion of a term. Rather than imposing a syntax on terms, we keep them abstract by stipulating only some basic properties. With this, we further develop a semantic framework for hybrid ASP solving and provide aggregate functions for theory variables that adhere to different semantic principles, show that they generalize existing aggregate semantics in ASP and how we can rely on off-the-shelf hybrid solvers for implementation.

==> aggregates-clingo.tex <==
\section{Capturing Constraint Aggregates in clingo} % $\mathit{HT}_{cc}$
\label{sec:aggregates-clingo}

\begin{itemize}
\item In the previous section,
we have introduced a general framework for dealing with condition-free aggregates and introducing some simple examples of how this framework can be instantiated.

\item In practice, things are slightly more complex.
For instance, continuing with our running example, it may be possible that our database wrongly assigns a non-integer to some person.
As a simple case assume that our database only has two people whose assigned savings are
$sav(p_1) = 1000$ and $sav(p_2) = \text{``error''}$.
This immediately falsifies the aggregate in rule~\eqref{eq:savings.fun.simpl} when its semantics is given by the function~\eqref{eq:sum.sem.simple}.
Note that $1000 +  \text{``error''}$ is mathematically not well-defined and it is evaluated as $\undefined$ by $\widehat{sum}$.
Note also that $\undefined \leq t_0$ is not true for any $t_0$.


\item In fact, the strategy followed by \texttt{clingo} consists in ignoring all non-integer values in aggregates. We may achieve this behaviour by applying an appropriate rewriting before applying the function $\widehat{sum}$.
That is, we define a new function
\begin{gather}
\widehat{sum}_\texttt{cl}(g) \eqdef \widehat{sum}(\texttt{cl}(g))
\end{gather}
where $\texttt{cl}(g)(i) = g(i)$ if $g(i) \in \mathbb{Z}$; and $\texttt{cl}(g)(i) = 0$ otherwise.
Now the same rule results on the sum $1000+0=1000$.
As a further example, consider the rule
\begin{gather}
p(1) \leftarrow sum\{ X : p(X) \} \geq 0
  \label{eq:ferraris}
\end{gather}
which under Ferraris semantics has the unique answer set~${ p(1) }$.
Assuming that $p(X)$ is true at most for one unique value, we can rewrite this rule in our framework as
\begin{gather*}
x = 1 \leftarrow sum\{ x \} \geq 0
\end{gather*}
Similarly, this rule has a unique equilibrium model where $x = 1$.

Recall that under Gelfond and Zhang's semantics rule~\eqref{eq:ferraris} has no stable models.
We can achieve a similar behaviour defining the following function
\begin{gather}
\widehat{sum}_\texttt{gz}(g) \eqdef \widehat{sum}(\texttt{gz}(g))
\end{gather}
where $\texttt{gz}(g)(i) = g(i)$ if $g(i) \in \mathbb{Z} \cup \{ \undefined \}$; and $\texttt{gz}(g)(i) = 0$ otherwise.
Note that
$\texttt{cl}$ can be defined in terms of
$\texttt{gz}$ as follows:
$\texttt{cl}(g) = \texttt{gz}(\texttt{rem}_{sum}(g))$
where
\begin{gather*}
\texttt{rem}_f(g)(i) = \begin{cases}
g(i) &\text{if }g(i) \neq \undefined\\
0_f  &\text{otherwise}
\end{cases}
\end{gather*}


\begin{proposition}
Given a stratified logic program~$P$,
let $P'$ be the result of replacing some aggregate atom of the form
\mbox{$f\langle t_1,\dots,t_n\rangle \prec t_0$}
by
\mbox{$g\langle t_1,\dots,t_n\rangle \prec t_0$}
such that $\hat{f} = \hat{g} \circ \texttt{\emph{rem}}_f$
and $0_f = 0_g$.
Then, $P$ and $P'$ have the same equilibrium models.
\end{proposition}

\end{itemize}






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> splitting.tex <==
\begin{itemize}
 \item


 \item
  To prove that Gelfond-Zhang and Ferraris semantics coincide for programs that are
  \emph{recursively \mbox{condition-free}}
  we will make use of the more general notions of supported model and splitting we introduce next.

 

\end{itemize} 


==> support.tex <==
\begin{itemize}
 \item 
  It is worth to mention that for standard ASP, it is known that Gelfond-Zhang and Ferraris semantics for aggregates coincide when the programs do no contain recursive aggregates.
  We show next that this is also the case in our generalisation to conditional constraint atoms.

 \item
  Let us start by defining the concept of logic program.
  A \emph{literal} is a constrain atom~$c \in \mathcal{C}$ or its default negation~$\neg a$.
  A \emph{rule} is a formula of the form $\varphi \leftarrow \psi$ where $\varphi$ and $\psi$
  respectively are a disjunction and a conjunction of literals
  called the head and the body of the rule.
  We assume that all non-negated constraints atoms occurring in the head of a rule are condition-free.
  By $\Head(r)$
  and
  $\Body(r)$
  we respectively denote the set of literals occurring in the head and the body of $r$.
  Furthermore, by $\Headp(r)$ (resp. $\Headn(r)$), we denote the set of positive (resp. negated) literals in $\Head(r)$.
  That is, $\Head(r) = \Headp(r) \cup \{ \neg c \mid \neg c \in \Headn(r) \}$.
  If clear from context, we write $\Body(r)$ for the conjunction of literals in the body,
  and $\Head(r)$ (resp. $\Headp(r),\Headn(r)$) for the disjunction of literals in the head (resp. positive, negative head ).
  For instance, $\tuple{h,t}\modelss \Body(r)$ stands for $\tuple{h,t}\modelss \bigwedge\limits\displaystyle_{l\in\Body(r)}l$ for interpretation $\tuple{h,t}$ and rule $r$.
  By
  $\Cond(r)$, we denote the set of variables occurring in a condition in some literal in~$r$.
  Note that $\Cond(r) \subseteq \vars{\Body(r)}$.
  A \emph{logic program} is a finite set of rules.
  A program is called \emph{condition-free} if all atoms occurring in it are condition-free.

   \item 

  
\end{itemize}


